PIXAL: Anomaly Reasoning with Visual Analytics

Anomaly detection remains an open challenge in many application areas. While there are a number of available machine learning algorithms for detecting anomalies, analysts are frequently asked to take additional steps in reasoning about the root cause of the anomalies and form actionable hypotheses that can be communicated to business stakeholders. Without the appropriate tools, this reasoning process is time-consuming, tedious, and potentially error-prone. In this paper we present PIXAL, a visual analytics system developed following an iterative design process with professional analysts responsible for anomaly detection. PIXAL is designed to fill gaps in existing tools commonly used by analysts to reason with and make sense of anomalies. PIXAL consists of three components: (1) an algorithm that finds patterns by aggregating multiple anomalous data points using first-order predicates, (2) a visualization tool that allows the analyst to build trust in the algorithmically-generated predicates by performing comparative and counterfactual analyses, and (3) a visualization tool that helps the analyst generate and validate hypotheses by exploring which features in the data most explain the anomalies. Finally, we present the results of a qualitative observational study with professional analysts. These results of the study indicate that PIXAL facilitates the anomaly reasoning process, allowing analysts to make sense of anomalies and generate hypotheses that are meaningful and actionable to business stakeholders.

==> chapters/casestudies.tex <==
% \begin{figure*}[hbt!]
%  \centering
% % \includegraphics[width=12cm]{pixal_figure.pdf}
% % \includegraphics[width=50mm,scale=0.5]{method.eps}
%  \includegraphics[width=100mm, scale=0.5]{chapters/final_images/sensors_high.png}
%  \vspace{-2em}
%  \caption{{\sys}: Sensors}
%  \vspace{-0.5em}
%  \label{fig:systemoverview}
% \end{figure*}


\section{Case studies}\label{sec:casestudies}
\begin{figure}[h]
 \centering
 \includegraphics[width=6cm]{chapters/final_images/second_vertical.png}
 \caption{\alg Sensor data - High temperature outlier}
\label{fig:pipeline}
\end{figure}
\begin{figure}[h]
 \centering
 \includegraphics[width=6cm]{chapters/final_images/second_vertical.png}
  \includegraphics[width=6cm]{chapters/final_images/first_vertical.png}
 \caption{\alg Sensor data - High temperature outlier}
\label{fig:pipeline}
\end{figure}
%To evaluate the effectiveness of \alg and our visual analytics tool we go through two case studies with real world data.
In addition to the two evaluations, we present two use cases of \alg to demonstrate the generalizability of \alg. Case study 1 showcases the use of \alg for analyzing temporal data, and case study 2 focuses on the analysis of a high-dimensional dataset.

\subsection{Case 1: Sensor Data}

The Intel Sensor Dataset is a set of sensor measurements collected from 54 sensors deployed in the Intel Berkeley Research lab between February 28th and April 5th, 2004. Each sensor is assigned an ID (moteid) and collects temperature, humidity, light, and voltage. Additionally, each measurement comes with a timestamp. We consider a scenario where an analyst is interested in locating anomalies in temperature.

Since the analyst knows they are primarily interested in the temperature feature, their first step is to select temperature from the barcode view (R1).
Upon inspecting the 1D subspace (R2) they notice that there are two anomalous clusters one at each extreme of temperature (-35 and 120).
Assuming that these will be explained by different factors, the analyst brushes over the anomalies with high temperature first. This generates the following predicates:

\begin{enumerate}[topsep=3pt, itemsep=0pt,parsep=3pt]
\item {(temperature $=$ 122.153)}
\item {(moteid $=$ 15) and (2004-03-02 07:40:59 $<$ dtime $<$ 2004-03-02 23:59:59)}
\item {(2.27 $<$ voltage $<$ 2.33)}
\item {(moteid $=$ 15) and (-1854.52 $<$ humidity $<$ 17.29)}
\item {(0.018 $<$ voltage $<$ 2.36) and (2004-03-02 07:40:59 $<$ dtime $<$ 2004-03-02 23:59:59)}
\end{enumerate}

\begin{figure}[H]
 \centering
% \includegraphics[width=12cm]{pixal_figure.pdf}
 \includegraphics[width=5.5cm]{chapters/final_images/sensorslow_vertical.png}
 \caption{\alg Sensor data - Low temperature outlier}
\label{fig:pipeline}
\end{figure}

By inspecting each predicate in the context of the rest of the data (R3), the analyst can come to the following conclusions:
\begin{enumerate}
\item The temperature is always exactly the same, likely a failure rather than an actual temperature
\item Sensor 15 failed during a specific time range
\item Voltages between 2.27 and 2.33 were only recorded when a sensor failed, therefor voltages in this range indicate failure
\end{enumerate}
Next the analyst brushes over the low temperature anomalies and generates the following predicates:
\begin{enumerate}[topsep=3pt, itemsep=0pt,parsep=3pt]
    \item {(-38.4 $<$ temperature $<$ -36.78)}
    \item {(-21.30 $<$ humidity $<$ -2.00)}
\end{enumerate}



Inspecting the low-temperature predicates, the analyst can come to the following conclusions:
\begin{enumerate}
    \item There were some very cold measurements between -38 and -36 degrees. Not clear from just this whether these are real or the results of sensor failure
    \item humidity is measured between 0 an 100, so ranges between -21.30 and -2.00 must have been there result of sensor failure. Conclude that the low anomalies are due to sensor failure not actual cold weather.
\end{enumerate}

\subsection{Case 2: Satellite Data}

Thirty-six features extracted from satellite observations with the goal of finding anomalies in soil images. In this scenario we assume that the analyst has no prior information about the data set suggesting where they should look first.
Looking at the barcode view, the analyst identifies that the set of features with the greatest number of anomalies is all features combined (R1).
Features are projected to two dimensions and plotted (R2). Looking at this plot the analyst observes that there is a cluster of points that is separated from the rest of the data (see Figure \ref{fig:systemoverview} B).
The analyst brushes over this cluster, generating the following predicates:
\begin{enumerate}
\item {(29.0 $<$ F33 $<$ 40.03)}
\item {(29.0 $<$ F21 $<$ 37.36)}
\item {(27.0 $<$ F17 $<$ 37.44)}
\item {(119.65 $<$ F35 $<$ 154.0)}
\item {(29.0 $<$ F29 $<$ 37.36)}
\end{enumerate}
Despite being given an unfamiliar data set, the analyst was able to use \alg to quickly generate a set of features and value ranges to explore. The analyst can now view each predicate (R3) to see the range of feature values in relation to the rest of the data and kickstart their analysis.
\begin{figure}[H]
 \centering
% \includegraphics[width=12cm]{pixal_figure.pdf}
 \includegraphics[width=6cm]{chapters/final_images/satellite_vertical.png}
 \caption{\alg Satellite }
\label{fig:pipeline}
\end{figure}




==> chapters/designstudy.tex <==
\section{Design Study} \label{ref:designstudy}

We have identified the following requirements for explainable anomaly detection. These requirements are based on interviews and continuous feedback from data analysts who are regularly tasked with generating actionable insights from anomaly detection approaches. In order to assure domain-independence and generalizability, we continuously reconciled our findings with the related work. In particular, we conducted structured interviews with six members of a data science and analytics team at a technology company providing driver assistance services to automotive and auto insurance brands.
Within this company, these selected personnel are primarily responsible for generating actionable reports from anomaly detection results after using off-the-shelf tools to analyze a large amounts of temporal transaction data. Our interview sessions lasted 30 minutes and were conducted over video conference due to the COVID-19 quarantine. With the consent of the participants, the audio portion of the interview was recorded. During the interviews, each participant was asked a set of questions designed to ascertain their overall familiarity with anomaly detection, any problems related to anomaly detection encountered during their job duties, and any existing tools or techniques that they have used for anomaly detection. Experts were then asked to outline their anomaly detection workflow.

\begin{itemize}
  \item \textbf{Goal G1 - Classify anomalies:} The primary goal of anomaly detection is to be able to correctly classify data points as either anomalies or normal points. This includes maximizing the percentage of points correctly classified as anomalies (true positive rate) and the percentage of points correctly classified as normal points (true negative rate). Additionally, we should minimize the percentage of normal points incorrectly classified as anomalies (false positive rate) along with the percentage of anomalies incorrectly classified as normal (false negative rate). These four metrics are commonly combined as an F1 score that ranks highly algorithms that balance precision and recall.
  \item \textbf{Goal G2 - Local explanation:} All data scientists mentioned the need to validate anomaly detection results by hand selecting representative data points and observing whether or not they were determined to be anomalies; both for understanding the model themselves and providing clarity for stakeholders. Additionally, many of the interviewed data scientists mentioned the need to compare points that were determined to be anomalies with similar points that were determined to be normal. Both of these needs fall under a need to provide local explanations for anomaly detection, or explanations for the classification of individual points.
  \item \textbf{Goal G3 - Global explanation:} The final and most important step of anomaly detection as laid out by interviewed data scientists was communicating the logic of the anomaly detection algorithm to business stakeholders. This includes both being able to summarize the logic of an algorithm and using business knowledge to explain the results in terms of relationships between variables. Only by putting the results of the anomaly detection algorithm in terms business stakeholders understand can the results of the algorithm be transformed into actionable insights.
\end{itemize}

We distill these goals into the following tasks that our system must be able to support to allow data users to perform explainable anomaly detection.

\begin{itemize}
  \item \textbf{Task T1 - Visualize explanations and compare multiple explanations:}
  Users in anomaly detection tasks are often faced with many competing alternatives, both in the choice of anomaly scoring algorithm and in explanations describing anomalies. Our tool must allow the user to quickly compare the feature space and performance of multiple explanations [G1].
  
  \item \textbf{Task T2 - Visualize relationships between variables for anomalies and non-anomalies:}
  In order create actionable insights from detected anomalies, analysts must be able to contextualize anomaly detection results in terms of variables in the dataset. Our tool must allow the user to contextualize generated explanations in relevant data attributes [G3].
  
  \item \textbf{Task T3 - Explain why an anomaly was flagged:}
  Validating anomaly detection results requires being able to inspect individual data points and whether they have been classified correctly. Our system must allow the user to inspect individual points and provide local explanations for why or why not they were included in a given explanations [G2].
\end{itemize}

==> chapters/goalsandtasks.tex <==
\section{Goals and Tasks} \label{ref:goalstasks}

The motivation for designing a visual analytics system on top of \alg is to help analysts to identify and make sense of anomalies and subsequently generate actionable data-insights, e.g., counter measures for network intrusion attacks or improvement suggestions for sensor networks. 
We are convinced that although many sophisticated automatic anomaly detection approaches exist, the solution for a sustainable and trustworthy anomaly detection lies at the intersection between automated and interactive approaches. 
Consequently, we asked ourselves which of the analysis steps can be linked and improved (a) algorithmically and (b) visually.

In our studies, we found that data scientists and analysts typically struggle not with finding anomalies, but choosing from the various possible root causes that led to an anomaly and communicate its impact and improvement suggestions. 
In particular, we conducted structured interviews with four data scientists and four data analysts at a large logistics company in the automotive domain.
Within this company, this personnel is primarily responsible for generating actionable reports from anomaly detection results after using off-the-shelf tools to analyze a large amounts of temporal transaction data. \mib{@brian: we have several times the analysts versus scientist distinction,  but this is uncommon in our field. Either we kill it or add one sentence about the diff here}. 
Our interview sessions lasted XXXX and were conducted over video conference due to the COVID-19 quarantine \remco{@brian: fill in}. 
With the consent of the participants, the audio portion of the interviews was recorded.
During the interviews, each participant was first presented with a set of xxx questions targeted on xxx and then was asked to outline his/her xxx workflow and then blah blah blah -- \remco{@brian: fill in the procedure}.

We analyzed and consolidated the results amongst the interview sessions to (a) identify the common workflows and (b) retrieve the specific (sub-)tasks that they are most struggling with in the automatic and visual analysis. 
We found that their workflow consists of the following steps: (1) researching appropriate features to include in an anomaly detection model, (2) validating anomalies generated by the model, and (3) presenting results to business stakeholders in a way that they are able to inform decisions. While this, in general, was not surprising and similarly reflected in recent work~\cite{Xu2020CloudDet, Cao2017Viola, Zhao2014FluxFlow}, we also found that the steps 1 and 2 often are deemed unsatisfactory by the business stakeholders. Data scientists and analysts are regularly questioned to check potential other root causes or alternative explanations--they were unaware off--for a problem, thus leading to a (time-consuming) feedback loop. 

Our work tackles the following challenges and domain goals analogous to the three working steps outlined above:
Within this workflow, the most common three goals reported by the participants are:

\noindent \textbf{Goal G1 - Retrieve expressive features without limiting the explanation possibilities:} Most HD data sets
% %, especially when derived from (virtual) sensors, 
are monitoring an impressive spectrum of feature dimensions. However, during the analysis the domain expert will quickly reduce the complexity by ignoring highly correlated, low-quality, or biased dimensions (G1a) and partition the dimensions into semantically linked subspaces (G1b). Both, sub-goals can be solved algorithmically, but only with caveats which inevitably require human inspection: For instance, the initially 30 dimensions of the Wine dataset were reduced to 14 by ignoring dimensions with acquisition artifacts and selecting one of two highly-correlated dimensions. However, 
% %if we leave the impact of  threshold decisions aside, 
while data quality is an partially objective measure, the choice between two dimensions are holding the same information content is arbitrary and should be guided by the dimension's natural explainability.
% %Data quality and information content are  is not an objective measures, (b) if  the selection is 
Likewise, the allocation of dimensions to a logical and (at best) non-overlapping subspaces, e.g., dimensions hat describe only the wine's appearance versus its chemical properties, also have a tremendous influence on the explainability in a later data analysis. 

% \noindent \textbf{Goal G2 - Reduce set of anomaly candidates to manageable size:}
\noindent \textbf{Goal G2 - Accountable reduction of anomaly candidates sets:}
%Filter uninteresting/non-actionable anomalies:
Anomaly detection algorithms, independent of their technical details, result in a large number of anomaly candidates of which only few justify the effort to, e.g., update an entire subsequent data analysis pipeline. From a data analysis view point, the applied AD technique should be general enough to capture also future incidences, thus also affecting the false positive rate negatively. As a counter-measure, crude domain-independent performance metrics, such as the support, exist for algorithmically ranking the distinctiveness of a candidate with respect to its neighborhood. From a business point of view, however, separating the wheat from the chaff is requires linking the candidate's attributes to domain knowledge, i.e., \emph{analytic explainability}.
%two intertwined steps: (G2a) find interesting anomalies and (G2b) 

\noindent \textbf{Goal G3 - Gathering actionable insights:} G1 and G2 are necessary preconditions for translating anomalies into actions. However, not all explanations are equally well-suited for a call to action and analysts often compare, analyze, and choose from a set of \emph{multiple explanations} to (a) find the most convincing one, (b) the one with business impact, i.e., \emph{implication explainability}, and (c) to select one explanation that outlines suitable counter-measures, i.e., \emph{operational explainability}. 

%For instance, it does not make sense to update the firewall settings of millions of PCs only because an intruder randomly scanned a port for its vulnerability.  
%compare explanations from a set of possible causes. While for G2a various , G2b is highly domain-dependent and only be automated for in well-specified problem settings. 

% \add{The motivation for designing \sys to help analyst identify and make sense of anomalies stems from observations of data scientists and analyst struggle with this task.
% In particular we conducted informal interviews with four data scientists and analysts at a large logistics company in the automotive domain.
% Within this company, these data scientists and analysts are primarily responsible for generating actionable reports from anomaly detection results after using off-the-shelf tools to analyze a large amounts of temporal transaction data.}

% \add{Each of the interview sessions lasted XXXX \remco{@brian: fill in}. 
% With the consent of the participants, the audio portion of the interviews were recorded.
% During the interviews (conducted over video conference due to the COVID quarantine), each participant was first presented with blah blah blah and then asked to do blah blah blah -- \remco{@brian: fill in the procedure}.}

% \add{We analyzed and consolidated the results of the interview sessions. 
% First, we identify the common workflow shared by these data scientists and analysts. 
% In particular, their} workflow consists of the following steps: (1) researching appropriate features to include in an anomaly detection model, (2) validating anomalies generated by the model, and (3) presenting results to business stakeholders in a way that is able to inform decisions once results from steps 1 and 2 are deemed satisfactory. Interestingly, these steps are similar to those found in existing systems outlined in the related work \cite{Xu2020CloudDet, Cao2017Viola, Zhao2014FluxFlow}.

% %Over the course of this project, we had access to seven domain experts whose responsibilities include generating actionable insights from anomaly detection results. While their workflow is specific to the automotive domain, a generalizable workflow emerged from their responses. This workflow consists of the following steps: 1) researching appropriate features to include in an anomaly detection model 2) validating anomalies generated by the model 3) presenting results to business stakeholders in a way that is able to inform decisions once results from steps 1 and 2 are deemed satisfactory. Interestingly, these steps are similar to those found in existing systems outlined in the related work \cite{Xu2020CloudDet, Cao2017Viola, Zhao2014FluxFlow}.

% %Our work tackles the following challenges and domain goals for \sys analogous to the three working steps outlined above:
% \add{Within this workflow, the most common three problems reported by the participants are:}

% \remco{@michael: I'm trying to play up the importance of having \textbf{multiple} explanations that the user can compare, analyze, and choose from. Can that be integratd into Goals and Tasks? See my writing in the related work section on program synthesis}

% \noindent \textbf{Goal G1 - Filtering dimensions for explainable features} \brian{move to task, make more specific} Most HD data sets
% %, especially when derived from (virtual) sensors, 
% are monitoring an impressive spectrum of feature dimensions. However, during the analysis the domain expert will quickly reduce the complexity by ignoring highly correlated, low-quality, or biased dimensions (G1a) and partition the dimensions into semantically linked subspaces (G1b). Both, sub-goals can be solved algorithmically, but only with caveats which inevitably require human inspection: For example, the initially 30 dimensions of the Wine dataset were reduced to 14 by ignoring dimensions with acquisition artifacts and selecting one of two highly-correlated dimensions. However, 
% %if we leave the impact of  threshold decisions aside, 
% while data quality is an partially objective measure, the choice between two dimensions are holding the same information content is arbitrary and should be guided by the dimension's natural explainability.
% %Data quality and information content are  is not an objective measures, (b) if  the selection is 
% Likewise, the allocation of dimensions to a logical and (at best) non-overlapping subspaces, e.g., dimensions hat describe only the wine's appearance versus its chemical properties, also have a tremendous influence on the explainability in a later data analysis. 

% \noindent \textbf{Goal G2 - Select and validate only interesting anomalies} Anomaly detection algorithms, independent of their technical details, result in a large number of anomaly candidates of which only few justify the effort to, e.g., update an entire subsequent data analysis pipeline. However, separating the wheat from the chaff is particularly challenging if the data analysis is accountable for these decisions. Various performance metrics can be used to address this challenging problem. One standard way is to assess the distinctiveness of the candidate with respect to its neighborhood, i.e., its support, other options are \mib{!??!?!??!?!}
% %taking various considerations into account: (a) Similar performance, aka have the support to be generalized 

% \noindent \textbf{Goal G3 - Turn anomalies into actionable insights} G1 and G2 are necessary conditions for translating anomalies into actions. However, not all explanations are equally well-suited for a call to action. For instance, it does not make sense to update the firewall settings of millions of PCs only because an intruder randomly scanned a port for its vulnerability.  

We use these goals to compile a set of visualization and interaction tasks for anomaly explanation. The mapping of these tasks to goals is indicated by square brackets:

\noindent \textbf{Task T1 - Explore expressive features} by visualizing anomalies calculated from different feature subsets and allowing the user to select different subsets to include in the anomaly detection model. [G1]

\noindent \textbf{Task T2 - Compare anomalies with normal points} by visualizing a two-dimensional embedding of all of the selected features with labeled anomalies. [G2] 

\noindent \textbf{Task T3 - Update anomaly selection} by allowing the user to brush over points in the two dimensional embedding. [G2]

\noindent \textbf{Task T4 - Compare anomaly explanations} by allowing the user to toggle between different explanations expressed as statements of predicate logic. [G3]

\noindent \textbf{Task T5 - Contextualize explanations}  by visualizing the subset of data defined by each predicate in the context of other relevant data. [G3] need a link to zoom pls


==> chapters/predicatelogic.tex <==

\section{Predicate Logic for Explaining Anomalies}\label{sec:method}

In order to showcase our algorithmic and visual solutions for the outlined requirements, we designed \alg, an anomaly explanation system that helps analysts to identify and make sense of anomalies and subsequently generate actionable data-insights.
%, e.g., counter measures for network intrusion attacks or improvement suggestions for sensor networks. 
We are convinced that although many sophisticated automatic anomaly detection approaches exist, the solution for a sustainable and trustworthy anomaly detection lies at the intersection between automated and interactive approaches. %\shan{nice}
Consequently, our primary contribution focuses on algorithmic aspects (explained in this section) and also introduces novel visual encodings for explaining anomalies (see~\autoref{sec:visualization}).
% \strike{\sys is a Visual Analytics system, which targets an interactive human-in-the-loop exploration by linking algorithmic support provided by \alg and visualizations (illustrated in ~\autoref{sec:casestudies}). \brian{change this to appendix}}

%\mib{done: copied paragraph from Sec3} \remco{@brian: this section needs to connect with the previous -- we identified a set of goals and tasks, so the writing here needs to relate to those} 

% As we learned in our interviews, the primary goals of \replace{data scientists and analysts}{data analysts} are 
For illustration purposes, we begin by outlining a \emph{guiding use case}, which is loosely based on scenarios described by our interview participants and describe how \alg can help to generate interpretable explanations of anomalies using a technique we call \textit{predicate induction}. 
%sessions that typically requires data analysts to retrieve impactful anomalies (\textbf{R2}) and turn them into actionable insights \textbf{(R3)}
%explainable anomaly detection %\brian{check that we're being consistent in how we use \alg vs ``predicate induction''}.
The monitoring of financial data is a crucial duty for business intelligence teams in all in industries. For example, an unexpected drop in revenue that is not quickly identified, corrected or explained, can have long-lasting negative impacts on a business.
Identifying these issues is not an easy task. While an analyst might be able to notice a drop in sales by looking at an aggregated view of all sales data over time, producing an explanation requires looking at the data at a more granular level. This might include different retail locations, products, time periods and operating hours, or a combination thereof. Additionally, identifying the cause of a drop in sales might also require changes in other variables that could include a weather event, changes in the market, or changes in staffing.

% \subsection{Anomaly Detection Algorithms}
% \label{sec:ADmodels}
In order to automatically support anomaly analysis
% The previous steps are contingent on a model having been chosen and trained to be a good fit to normal data. While 
a number of learning algorithms have been proposed \cite{goldstein2016comparative}. Since choosing the right AD algorithm is challenging and depends on the use case, our explainability approach should require only the common denominator among all these techniques: a score describing the normalcy, respectively anomaly of data points. All state-of-the-art anomaly detectors, independent of their implementation details, allow us to derive this score. Probabilistic Gaussian approaches\cite{Rousseeuw1984MCD}, for instance, compute the negative log likelihood of a point given a covariance model of the data set. The Local Outlier Factor algorithm\cite{breunig2000lof} determines the normalcy of a data point by examining how isolated it is with respect to its neighbors based on the reachability distance. Isolation forest\cite{liu2008isolation} assigns an anomaly score to a point based on the number of splits needed to partition that point from the rest of the data.
While any of these algorithms might serve as a reasonable option for a generic data set, we recognize that this choice will not be appropriate for all data sets. One of the strengths of \alg, however, is that it is \emph{agnostic} to the chosen model: any set of parameters can be used to model a particular data set, provided that each point receives an anomaly score.
%that is i to its normalcy with respect to the model. 
% \subsubsection{Gaussian}
% Given no prior information about our data set $D$, the model that allows for the most uncertainty is a multivariate Gaussian. This model is defined by a mean vector, $\mathbf{\mu}$, of length $M$, and an $M \times M$ covariance matrix $\Sigma$. Since we expect that $D$ will contain anomalies, we use a robust approximation for these parameters. For the vector of means, we can take the median value of each feature. To approximate the covariance matrix, we use minimum covariance determinant method\cite{Rousseeuw1984MCD}, which finds $\frac{N + M + 1}{2}$ data points whose empirical covariance has the smallest determinant. Given our estimates of $\mathbf{\mu}$ and $\Sigma$, the anomaly score is simply the negative log likelihood given by:
% \begin{equation}
%     \log P(D|\mu, \Sigma) = - \frac{N}{2} \log |\Sigma| - \frac{1}{2} \sum_{x \in D} (x - \mathbf{\mu})^{\top} \Sigma^{-1} (x - \mathbf{\mu})
% \end{equation}

% \subsubsection{Local Outlier Factor}
% One method of determining the normalcy of a data point is by examining how isolated it is with respect to its neighbors. The local outlier factor\cite{breunig2000lof} of a point is determined by first computing its local reachability distance (LRD) to its $k$ nearest neighbors:
% \begin{equation}
% LRD_{k}(x) = 1 / \frac{\sum\limits_{o \in N_{k}(x)} d_{k}(x, o)}{|N_{k}(x)|}
% \end{equation}
% where $d_{k}(x, o)$ is the reachability distance between the neighboring point $o$ and $x$. The Local Outlier Factor (LOF) is then computed by taking the ratio of the LRD values for each neighbor of $x$ and the LRD of $x$ itself:
% \begin{equation}
% LOF(x) = 1 / \frac{\sum\limits_{o \in N_{k}(x)} \frac{LRD_{k}(o)}{LRD_{k}(x)}}{|N_{k}(x)|}
% \end{equation}
% \strike{While there are extensions of this algorithm that normalize LOF to be a probability, our method only requires that the score assigned to the points be proportional to a log likelihood. Therefore, when using this algorithm for predicate induction we can simply use the LOF as a proxy for log likelihood.} \brian{taking out since I go over this in 4.1}

% \subsubsection{Isolation Forest}
% Random forests are a common way for partitioning instances belonging to different classes by recursively selecting features and a split value. Isolation forests\cite{liu2008isolation} borrow this procedure for assigning anomaly scores to instances, observing that anomalous points will require fewer splits to partition away from the rest of the data set. For a tree of height $n$, the anomaly score for the point $x$ is given by
% \begin{equation}
% s(x, n) = 2^{\frac{-E(h(x))}{c(n)}}
% \end{equation}
% where $c(n)$ is the average path length of an unsuccessful search in a BST of height $n$ and $E(h(x))$ is the average from a collection of isolation trees.




Using predicate induction, explanations for anomalies can be automatically determined using the following steps. First, we split features of the data set into \textit{target} features (sales) and \textit{context} features (e.g., region, product, weather). 
%\brian{I don't think we mention context features anywhere else in the paper}. 
Next, we are training an anomaly detection model on the target features, generating anomaly scores for each data point in the data set. Finally, we use an iterative algorithm to generate a set of predicates whose bounding boxes enclose data points with high anomaly scores in terms of both their target and contextual feature values. In our sales example, we train an anomaly detection model on the \textit{sales} target feature that we use to assign each instance an anomaly score. We then find a set of logical statements based on the context features \textit{date, region, weather}, such as \textit{date is between January 20th and January 30th, location is northeast, weather is snowy}, that separate anomalous points from normal points when applied to the data set. By visualizing these predicates in the context of the full data set, the user is able to draw conclusions about the mechanisms that led to a drop in sales, e.g., shoppers in the northeast stayed home during a winter storm that occurred at the end of January.

% For an input dataset where some subset of points are anomalies, our goal is to separate the anomalous points from the "normal" points in a way that is human understandable. One approach is to generate statements of predicate logic that filter out the anomalies when applied to the dataset. Predicates in conjunctive normal form consist of a set of clause connected by \textbf{AND}, where each clause is a set of Booleans connected by \textbf{OR}. Restricting each clause to operate on only one column of the dataset, a clause on the $k-th$ column will be of the form $p^{k}(x_{i}) = f^{1}(x^{k}_{i},y_{1}) \vee f^{2}(x^{k}_{i},y_{2}) \vee ... \vee f^{m}(x^{k}_{i},y_{m})$ where $f^{m}$ is a Boolean function. If the $k-th$ column is continuous then $f^{m}(x^{k}_{i},y_{m}) \in \{x^{k}_{i} > y_{m}, x^{k}_{i} < y_{m}\}$. If the $k-th$ column is discrete then $f^{m}(x^{k}_{i},y_{m}) \in \{x^{k}_{i} = y_{m}\}$. The instance $x_{i}$ will be separated as an anomaly if $p(x_{i}) = p_{1}(x_{i}) \wedge p_{2}(x_{i}) \wedge ... \wedge p_{k}(x_{i})$ evaluates as true, allowing us to separate the full dataset $D$ into anomalies, $p(D) = \{x_{i} \in D | p(x_{i})\}$ and normal points, $\neg p(D) = \{x_{i} \in D | \neg p(x_{i})\}$.

% Using predicates as our basis for explaining anomalies, our goal is to find a set of predicates that effectively separates anomalies from normal points given a particular dataset. In this section we describe \alg, an algorithm for efficiently inducing this set of predicates.

\subsection{Predicate Influence}

Our use of predicates to describe anomalies is inspired by the Scorpion system developed by Wu et al.\cite{wu2013Scorpion}, which aims to reveal the influence of feature subpaces for outliers that would typical be (statistically) ``averaged out'' by common database aggregate queries. Their system takes a data set and an aggregate function as input and outputs a set of predicates whose bounding boxes enclose a set of points that have a high influence on the value that the aggregate function returns. The \textit{influence} of a predicate with respect to the function $y = f(x_{1}, x_{2}, ... , x_{n})$ is defined by $\frac{\Delta y}{\Delta x}$ or the change in the output given a change in the input. For a given aggregate function $agg$ the influence of predicate $p$ depends on the change in the aggregate after removing the set of data points enclosed by $p$ (represented as $p(D)$) from $D$:
\begin{equation}
    \Delta agg(D, p) = agg(D) - agg(D - p(D))
\end{equation}
The influence of $p$ with respect to $agg$ is then the change in the output of $agg$ given the change in the dataset:
\begin{equation} \label{eq:score}
inf_{agg}(D, p) = \frac{\Delta agg(D, p)}{|p(D)|}
\end{equation}
where $|p(D)|$ is the number of data points removed from $D$. We will now demonstrate how this formulation can be applied to generating multiple explanations for anomalies.

We define $\mathcal{M}$ to be a probabilistic model describing a data set $D$. For each data point $x$, its likelihood under $\mathcal{M}$, $P(x | \mathcal{M})$ describes how well the point is described by the model. In other words, ``normal'' points as defined by $\mathcal{M}$ will have a relatively high likelihood compared to anomalous points. To measure the overall ``normalcy'' of $D$ with respect to $\mathcal{M}$ we take the joint likelihood over all points in the data set:
\begin{equation}
P(D|\mathcal{M}) = \prod_{x_{i} \in D} P(x_{i}|\mathcal{M})
\end{equation}
Using this formulation we can measure the change in the joint likelihood under $\mathcal{M}$ that occurs from removing a set of points enclosed by the predicate $p$, $p(D)$:
\begin{equation}
P(D - p(D)|\mathcal{M}) = \frac{P(D | \mathcal{M})}{P(p(D)|\mathcal{M})}
\end{equation}
Alternatively, we can express the change in the relative ``normalcy'' of $D$ with respect to $\mathcal{M}$ after removing $p(D)$ in terms of the joint log likelihood of the points $p(D)$:
\begin{equation}
\Delta \mathcal{L}_{\mathcal{M}}(D, p) = - \log P(p(D)|\mathcal{M}) = \sum_{x_{i} \in p(D)} -\log P(x_{i}|\mathcal{M})
\end{equation}
We define the \textit{likelihood influence} as the change in the joint log likelihood of $D$ with respect to $\mathcal{M}$ that occurs when we remove the data points $p(D)$, per data point removed:
\begin{equation}
inf_{\mathcal{L}}(D, p) = \frac{-\log P(p(D)|\mathcal{M})}{|p(D)|}
\label{eq:normality}
\end{equation}

While not all anomaly detection algorithms explicitly define a likelihood function, most output a score for each data point meant to indicate the degree to which it is anomalous. In other words, most anomaly detection algorithms, probabilistic or not, output a score that is proportional to the negative log likelihood of some unknown probabilistic model that defines normal behavior. Since we are only interested in likelihoods and not normalized probabilities we loosen the definition of likelihood influence to be the change in the sum of anomaly scores:
\begin{equation}
inf_{\mathcal{L}}(D, p) = \frac{\sum\limits_{x_{i} \in p(D)} score(x_{i})}{|p(D)|}
\end{equation}

\subsection{Bottom-up search for Predicate Induction}
\label{sec:bottomup}
Here we describe a procedure for finding a predicate with the highest possible likelihood influence.
The bottom-up search starts with a set of single-feature predicates, each representing a slice of the data set along a single feature, and iteratively combines predicates until their likelihood influence stops increasing. This can be broken down into four steps:

\vspace{6pt}
\noindent \textbf{Initialize}: The first step is to generate all single-feature predicates. For discrete features, each predicate captures a single feature value, e.g., $City = Boston$. For continuous features the values are first discretized so that each each predicate represents a range, e.g., $31 \degree \text{F} < Temperature < 32 \degree \text{F}$.

\vspace{6pt}
\noindent \textbf{Merge}: We merge predicates by taking each predicate in order of likelihood influence and attempting to combine it with adjacent predicates (also in order of likelihood influence). Two predicates are merged if the likelihood influence of the merged predicate is greater than the likelihood influence of either original predicate. We merge discrete features by taking the union of the values, i.e., $merge(City=Boston, \, City=Chicago) = City \in \{Boston, Chicago \}$, and merge continuous features by computing the union of the two ranges, i.e., $merge(31 \degree \text{F} < Temperature < 32 \degree \text{F}, \, 33 \degree \text{F} < Temperature < 34 \degree \text{F}) = 31 \degree \text{F} < Temperature < 34 \degree \text{F}$.

\vspace{6pt}
\noindent \textbf{Intersect}: Following the merge step, we are left with a set of single-feature predicates. This step attempts to combine each pair of predicates that contain different features. As in the previous step, we intersect predicates if the likelihood influence of the intersected predicate is greater than the likelihood influence of either original predicate. Predicates are intersected by taking the conjunction of the original predicates, i.e., $intersect(City=Boston, \, 31 \degree \text{F} < Temperature < 32 \degree \text{F}) \rightarrow (City=Boston \, \wedge \, 31 \degree \text{F} < Temperature < 32 \degree \text{F}$).

\vspace{6pt}
\noindent \textbf{Prune}: The preceding intersect step takes the number of predicates from $n$ to a maximum of $\binom{n}{2}$ if we combine all pairs of predicates. The purpose of pruning is to reduce this number by removing any predicates that are unlikely to contribute to the eventual best predicate. We achieve this by first finding the most influential predicate so far, $p^{*}$, and identifying the point enclosed by $p^{*}(D)$ with the highest anomaly score.
We then remove all predicates that do not contain this point, as merging or intersecting any of these predicates with the current best predicate can only reduce its likelihood influence.

We repeat the merge, intersect, and prune steps and record the predicate with the highest likelihood influence at each iteration. This procedure terminates when the likelihood influence of the best predicate does not improve between the iterations. 
%at the current iteration is not greater than the likelihood influence of the best predicate at the previous iteration.

% Following the initialize step, the merge, intersect, and prune steps are repeated, recording the predicate with the highest likelihood influence at each iteration. This procedure terminates when the likelihood influence of the best predicate at the current iteration is not greater than the likelihood influence of the best predicate at the previous iteration.

We can introduce an additional strictness parameter, $c$, to modulate the penalty in likelihood influence incurred based on the number of points enclosed by a predicate:
\begin{equation}
inf_{\mathcal{L}}(D, p) = \frac{\sum\limits_{x_{i} \in p(D)} score(x_{i})}{|p(D)|^{c}}
\end{equation}
With this addition, lower values of $c$ will result in predicates that enclose more points overall, while $c=1$ will result in predicates that strictly minimize per-point anomaly score.

\subsubsection{Multiple explanations}
Oftentimes, anomalies have more than one reasonable explanation that could be operating either independently or in tandem with others. For instance, a decrease in sales could be due to two separate issues at two different store locations, or due to a local weather event, such as a snowstorm in the northeast. We allow the user to make use of multiple candidate explanations by adding an additional outer loop to the bottom-up search procedure. Rather than returning only the best predicate, the inner loop now returns both the best predicate and the set of remaining unused predicates. In every new iteration, we initialize the inner loop with the remaining predicates. Finally, the best predicate from the previous iteration and the best predicate from the new iteration are combined by taking the disjunction of the two, i.e., $disjunction(region = northeast, \, weather=snowy) = region = northeast \lor weather=snowy$. We continue this process until the likelihood influence of the conjunction of the current best predicate and the new best predicate is less than the likelihood influence of the current best predicate alone.

\subsubsection{Pruning with User Input}
We further reduce the size of the set of candidate predicates to increase performance with the help of the user. 
%by using insights the user may have about which points are anomalous. 
Given a set of points identified by the user as being anomalous, $x ^{\prime}$, we add an additional pruning step to the inner loop that  removes all predicates that do not include any of the points in $x^{\prime}$.

% \subsection{Anomaly Detection Algorithms}
% \label{sec:ADmodels}
% The previous steps are contingent on a model having been chosen and trained to be a good fit to normal data. While a number of learning algorithms have been proposed for anomaly detection \cite{goldstein2016comparative}, the best choice depends on the use case. With that said, we list here a few common algorithms that have demonstrated good performance across a variety of data sets, and can serve as a good starting place for \alg. % \shan{wait are we not going to list them?} \brian{(listed below)}

% \subsubsection{Gaussian}
% Given no prior information about our data set $D$, the model that allows for the most uncertainty is a multivariate Gaussian. This model is defined by a mean vector, $\mathbf{\mu}$, of length $M$, and an $M \times M$ covariance matrix $\Sigma$. Since we expect that $D$ will contain anomalies, we use a robust approximation for these parameters. For the vector of means, we can take the median value of each feature. To approximate the covariance matrix, we use minimum covariance determinant method\cite{Rousseeuw1984MCD}, which finds $\frac{N + M + 1}{2}$ data points whose empirical covariance has the smallest determinant. Given our estimates of $\mathbf{\mu}$ and $\Sigma$, the anomaly score is simply the negative log likelihood given by:
% \begin{equation}
%     \log P(D|\mu, \Sigma) = - \frac{N}{2} \log |\Sigma| - \frac{1}{2} \sum_{x \in D} (x - \mathbf{\mu})^{\top} \Sigma^{-1} (x - \mathbf{\mu})
% \end{equation}

% \subsubsection{Local Outlier Factor}
% One method of determining the normalcy of a data point is by examining how isolated it is with respect to its neighbors. The local outlier factor\cite{breunig2000lof} of a point is determined by first computing its local reachability distance (LRD) to its $k$ nearest neighbors:
% \begin{equation}
% LRD_{k}(x) = 1 / \frac{\sum\limits_{o \in N_{k}(x)} d_{k}(x, o)}{|N_{k}(x)|}
% \end{equation}
% where $d_{k}(x, o)$ is the reachability distance between the neighboring point $o$ and $x$. The Local Outlier Factor (LOF) is then computed by taking the ratio of the LRD values for each neighbor of $x$ and the LRD of $x$ itself:
% \begin{equation}
% LOF(x) = 1 / \frac{\sum\limits_{o \in N_{k}(x)} \frac{LRD_{k}(o)}{LRD_{k}(x)}}{|N_{k}(x)|}
% \end{equation}
% % \strike{While there are extensions of this algorithm that normalize LOF to be a probability, our method only requires that the score assigned to the points be proportional to a log likelihood. Therefore, when using this algorithm for predicate induction we can simply use the LOF as a proxy for log likelihood.} \brian{taking out since I go over this in 4.1}

% \subsubsection{Isolation Forest}
% Random forests are a common way for partitioning instances belonging to different classes by recursively selecting features and a split value. Isolation forests\cite{liu2008isolation} borrow this procedure for assigning anomaly scores to instances, observing that anomalous points will require fewer splits to partition away from the rest of the data set. For a tree of height $n$, the anomaly score for the point $x$ is given by
% \begin{equation}
% s(x, n) = 2^{\frac{-E(h(x))}{c(n)}}
% \end{equation}
% where $c(n)$ is the average path length of an unsuccessful search in a BST of height $n$ and $E(h(x))$ is the average from a collection of isolation trees.

% While any of these algorithms might serve as a reasonable choice for a generic data set, we recognize that this choice will not be appropriate for all data sets. One of the strengths of \alg is that it is agnostic to the chosen model: any set of parameters can be chosen to represent a particular data set, provided that each point can be given a score that is inversely proportional to its normalcy with respect to the model. 

==> chapters/visualinterface.tex <==
\begin{figure*}
 \centering
% \includegraphics[width=12cm]{pixal_figure.pdf}
 \includegraphics[width=\linewidth]{chapters/final_images/pixal_full.jpg}
 \vspace{-2em}
 \caption{A visual analytics system for \alg: In this anomaly analysis scenario the user selects an explanation to explore by a combination of overall score and features included (A). Anomalous points contained in the chosen explanation are then compared to adjacent non-anomalous points in the scatter plot view(B). To further evaluate the explanation, known anomalies or non-anomalies can be selected in the table view (C) to be highlighted in B. Finally, the user synthesises multiple explanations by viewing them together in the scatter plot view.}
 \vspace{-0.5em}
 
 %Panel A, the feature view, visualizes the data across features and feature combinations. The projection view in Panel B shows the user a T-SNE projection of their selected feature combination. Panel C is the explanation view. Each tab holds a generated predicate, and the tray contains the details about the those predicates. Finally, in the small-multiple panel D, to the right, users can examine the raw data across each feature included in the generated predicate, including the highlighted range where anomalies are likely to occur.}
 \label{fig:systemoverview}
\end{figure*}

\section{Visualizing Anomaly Predicates}\label{sec:visualization}
%\brian{connect back to tasks}
%\brian{start with high level workflow}
%\mib{ \dots; We will demonstrate the VA system according to the task pipeline outlined in ``Task and Goals''.}
One major design choice for \alg is to support the algorithmic analysis with visual means to infuse domain- and common knowledge into the process. Based on our requirement analysis (see~\autoref{ref:goalstasks}), we present in this section our visual solutions for data analysts in their main workflow steps comparing explanations (\textbf{R1}), comparing anomalies with similar non-anomalies (\textbf{R2}), synthesising multiple explanations (\textbf{R3}).
\autoref{fig:systemoverview} shows an overview of our visual analytics system, which consists of three panels: (A) \viewA, (B) \viewB, and (C) \viewC. 
In the subsections below, we describe each part of the visualization, their interactive features, and how they support the three system design requirements.

\subsection{Steering Interpretable Anomaly Detection through Visual Explanation Ranking (R1)}

\textit{``What makes a data point anomalous?''} In our interviews with the data scientists and analysts this question came up repeatedly without a satisfactory answer.
In high-dimensional data, every data point can be normal or anomalous depending on the subspaces in which the data point is considered.
These subspaces can be a single dimensional space or combinations of multiple dimensions.
Identifying what data points are anomalous and in which subspaces is often the first task that a data analyst tried to address.

\begin{wrapfigure}{R}{4cm}
\centering
\vspace{-1em}
\includegraphics[width=1.0\linewidth]{figures/featurebarcodes.png}
\vspace{-2em}
\end{wrapfigure}
To support the analyst in quickly identifying anomalous data points in subspaces, we designed the (A) \viewA, a barcode representation of the distribution of anomaly scores (for all data points) in a particular single and multidimensional subspace. 
%In this view, each subspace is a bar, representing all possible subspaces, including those that are .
A single data point is shown as a vertical line in dark gray, or what our team has referred to as a 'mark' on the barcode. A mark's position along the x-axis of the bar represents its anomaly score as computed using Equation~\ref{eq:score}.
%Data points with a low anomaly score are placed further to the left, whereas points found to be anomalous appear towards the right of the bar. 
All of the marks and the barcodes themselves are interactive allowing the user to inspect a single data point and visualize it across multiple subspaces. To inspect a range of data points, i.e., deem them anomalous, we introduce an interactive filter slider. If any barcode mark has a score above this threshold, it will appear on the barcode as orange. Otherwise, it will remain dark gray.

%Above the barcode chart is a slider UI. 
%Another interaction filter is the This slider determines the threshold above which a data point's x value (anomaly score) is deemed anomalous. 
%The user can interactively determine the threshold above which data points are deemed anomalous.

The \viewA shows a number of these bars, each representing a subspace.
As an offline, pre-computation process the \alg visualization enumerates all subspaces up to $\mathbb{R}^3$, resulting in $n + {n \choose 2} + {n \choose 3}$ number of rows, where $n$ is the number of features in the input data. This decision is informed by the data analysts we interviewed, but also helps in reducing the pre-computation time. While this restriction resembles an educated preselection, it can also be modified to fit the needs of analyst at any time.
These rows can be organized in different ways to help the analyst focus on the most relevant subspaces to examine.
For example, in \autoref{fig:systemoverview}, we sort the rows such that subspaces with the most anomalous data points appear first.

The \viewA affords two ways for analysts to begin their search for anomalies in a data set. 
First, to investigate a specific question or hypothesis, the analysts can search for a specific subspace and focus their investigation, e.g., investigate temperature anomalies in a sensor data.
%, the analyst would select the bar specific to the temperature feature in the data.

However, in the case where the analyst does not have a preconceived domain-question, the \viewA supports the visual exploration of the subspaces. %\mib{@brian/shannon describe how interesting barcodes look like: Check the following sentence! Important!}
Interesting anomaly barcodes will not only display higher anomaly scores, but also clearly separate their anomaly score ranges. Vice versa, uninteresting barcodes will resemble a dense low value region and can be easily neglected/filtered. %\brian{perfect}
%In \alg we currently limit the number of spaces to the combination of a maximum of three features.
% \shan{BA BAM.}

\subsection{Viewing explanations in context (R2a) and synthesizing explanations (R3}

%\mib{can we have the same guiding quesiton here:}
\textit{``How do anomalous data point compare to normal points?''}
Once the analyst has selected the subspace of interest, the data points are displayed in the \viewB.
Depending on the dimensionality of the chosen subspace the scatterplot view changes its axes encoding. 

\begin{wrapfigure}[]{R}{3.5cm}
\centering
\vspace{-1em}
\includegraphics[width=1.0\linewidth]{three_scatter.png}
\vspace{-2em}
\end{wrapfigure}
If the subspace only has one dimension, the anomaly scores of the data points will be selected as the x-axis and the raw data values used as the y-axis.
When the subspace has two dimensions, each of the dimensions is used as the x- or y-axis.
Lastly, when the subspace has three (or more) dimensions, we use t-SNE to project the data points into 2D, at which point the axes are no longer meaningful. In the case of Figure 2, the selected subspace is multidimensional.
Consistent with the other views, data points are colored in grey if their anomaly score is below the user-selected threshold and orange if above. The orange points on the projection view are the same points identified in orange on the barcode view. This coordinated data point identification is helpful for data scientists to thread a story through their explanation as to what might be the root cause of these anomalies.

While the \viewB serves as a way to visualize the anomalous data as it relates to the normal (\textbf{R2}), it also serves as a way to perform interactive model-sensibility analysis (\textbf{R3}).
\begin{wrapfigure}{R}{5.5cm}
\centering
\vspace{-1em}
% \includegraphics[width=1.0\linewidth]{figures/bar_and_scatter.png}
\includegraphics[width=1.0\linewidth]{figures/sensibilityanalysis.png}
\vspace{-2em}
\end{wrapfigure}
Adding or removing anomalous points (blue selection in top subspace), based on the analysts' domain knowledge, is an often requested feature (in our interviews) that we learned is oftentimes not (even) supported by off-the-shelf commercial products. 
As noted by these analysts, before they commit to investigating the cause of an anomaly, they must be able to first confirm that the algorithm is producing reasonable candidates.
The brushing selection allows the analyst to perform this task in a ``non-commital'' manner--that is, since the analyst can quickly and easily add or remove anomalies from the algorithm's recommendation, they are not bound by the limits of of the algorithm.

They are instead, free to reassure if their domain knowledge is reflected in the data to gather a set of anomalies that reflect their belief and understanding, as well as the analysis context. This also helps to address the other noted work flow constraint of having to reproduce time-consuming work upon additional suggestions from stakeholders.

\subsection{Inspecting Individual Points (R2b)}
\label{sec:vis:r3}
%\brian{break into easy, hard, and multiple explanations}

\textit{``Can I translate this anomaly into an action (with business impact)?''}
\begin{wrapfigure}[]{R}{6.2cm}
\centering
\vspace{-1.5em}
 \includegraphics[width=1.0\linewidth]{figures/anomalyexplanationview}
\vspace{-2em}
\end{wrapfigure}
After the analyst has finalized the set of anomalous data points, we execute the \alg algorithm described in \autoref{sec:bottomup} to generate explanations.
Our resulting (multiple) explanations get separated into ``tabs'' displayed in the \viewC.
%where each explanation gets a separate ``tab'' in the panel.
Each tab contains a human-readable, textual representation of the predicates that make up the explanation.
Distinguishing ``actionable'' or ``interesting'' explanations is certainly a human task. With \alg, though, we can take advantage of our normality quality metric (described in \autoref{eq:normality}) to rank and order explanations.  
To further facilitate this task, we added details-on-demand through number of visualizations in the \viewD, where each view corresponds to a data feature in a predicate.
In each of these small-multiples, the range of a predicate is colored with an orange band, indicating the bounds between which PIXAL has identified this feature variable as contributing to anomalous data points.


%For example, in Figure~\ref{fig:small-multiple}, the selected predicate (Predicate 1) shows that values between 30 and 40 for the 33rd feature variable are found to indicate potential cause of the anomalies. \shan{Would it be more helpful to describe all this in the context of the example data sets we used? I have been wondering why that haven't been mentioned yet. These images show the satellite data sets but I can quickly change them to show the sensor one instead if we think that's meatier.}
The combination of the \viewC and \viewD allows the analyst to explore and compare the explanations in a number of ways.
First, it supports the analyst to dig deep into the analysis of an explanation.
Specifically, as described in \autoref{sec:bottomup}, \alg uses a bottom-up approach to identify the relevant predicates. Operations, such as \textbf{merge} and \textbf{prune}, seek to maximize the log likelihood while also minimizing the number of predicates.
In doing so, the resulting set of predicates can end up including or excluding data points from the set of anomalous points as originally identified by the analyst.
For instance, in the \textbf{merge} example in \autoref{sec:bottomup}, two predicates, $(31 \degree \text{F} < Temp < 32 \degree \text{F})$ and $(33 \degree \text{F} < Temp < 34 \degree \text{F})$ are combined into a single one: $(31 \degree \text{F} < Temp < 34 \degree \text{F})$, which on the one hand reduces explanation's complexity, but also reduces the predicate's specificity (a domain- and task-dependent trade-off). 
%However, notice that in doing so, data points for which the temperature readings are between 32 and 33 are inadvertently included as anomalous. \shan{add a 'so what'. what is the implication of this last statement?}


% \begin{wrapfigure}{R}{5.5cm}
% \centering
% % \vspace{-1em}
% \rule{3cm}{5.5cm}
% % \vspace{-2em}
% \end{wrapfigure}
Our \viewD serves another purpose: It allows the analyst to reexamine the raw data without the effects of an algorithmic intervention, i.e., to verify that anomalous data points are in fact outlying.
When used in conjunction with the \viewC the analyst can quickly jump back and forth between different explanations and compare the overall effects of distinct explanation facets and test potential intervention paths (\textbf{R3}).
It is relevant to note that the comparison does not necessarily have to result in selecting one ``best'' explanation.
Instead, as we describe in \autoref{sec:eval:qualitative}, we found that analysts often form a higher-level understanding of the root cause of an anomaly from examining \textit{all} explanations. 
%that any single explanation will not be able to describe.

%The \viewD serves as a mechanism to help the analyst visualize the effects of these predicates and identify data points that are mistakenly included or left off from the initially identified list of anomalies. It also helps data scientists to verify that anomalous data points are in fact, outlying. 
%Though the data is visualized in a variety of different ways across the four views of the PIXAL interface, it is clear that there is consistency in what is being identified as anomalous across all forms. Those barcode marks identified as orange on view A are the same included in the cluster brushed in view B, are the same as those segments of the small multiple charts that fall within the yellow bands. Furthermore, the fully linked interactions allow for complete exploration and comprehensive understanding of what the PIXAL algorithm has presented to the user. In this way, the interface is a one-stop-shop for establishing trust between the domain user, the data, and the model.
%\shan{I kind of rambled here... it's late, can someone peep this for relative sanity?}


% \begin{figure}[hbt!]
%  \centering
%  \includegraphics[width=6cm]{pixal_predicates.pdf}
%  \includegraphics[width=6cm]{pixal_plot.pdf}
%  \caption{The explain view lists out the various feature ranges included in the selected predicate. This particular view shows that PIXAL has generated five predicates for found anomalies. The data range for the feature (feature 33) in the currently selected predicate (Predicate 1) is visualized as the yellow band.}
% \label{fig:small-multiple}
% \end{figure}
